The Tropical Superpotential For $\mathbb{P}^2$

We present an extended worked example of the computation of the tropical superpotential considered by Carl--Pumperla--Siebert. In particular we consider an affine manifold associated to the complement of a non-singular genus one plane curve, and calculate the wall and chamber decomposition determined by the Gross--Siebert algorithm. Using the results of Carl--Pumperla--Siebert we determine the tropical superpotential, via broken line counts, in every chamber of this decomposition. The superpotential defines a Laurent polynomial in every chamber, which we demonstrate to be identical to the Laurent polynomials predicted by Coates--Corti--Galkin--Golyshev--Kaspzryk to be mirror to $\mathbb{P}^2$.

==> drafts.tex <==

%In the proof of Theorem~\ref{thm:superpotential} we will make use of a gluing construction, in which $\Diag(P,v,k)$ is created from gluing together diagrams $\Diag(P_i,v_i,1)$ for sequences of polygons $P_i$ and vertices $v_i$. Indeed, given a diagram $\Diag(P,v,k+1)$, and $i \in \{1,2\}$, the triangular region $\fu^i_k$ is mapped to a (unique) Fano polygon $P^i_k$ by a suitable scale and translation $S_i$. Let $v^i_k$ denote the vertex of $P^i_k$ such that the corresponding vertex of $\fu^i_k$ is not contained in $\fu_{i,j}$ for any $j < k$. Consider the diagram $\Diag(P^i_k,v^i_k,1)$ and -- to avoid duplicating notation -- let $\bar{\fu}^i_1$ and $\bar{\fu}_0$ denote the triangular regions defined by this embedded simplicial complex in $\R^2$, labelled as above. This construction is shown in Figure~\ref{fig:gluing_diagrams}, and we record the following simple -- but important -- Lemma.



%Fix a triple $(P,v,k)$ where $P \subset N_\R$ is a Fano polygon $P$ with singularity content $(3,\emptyset)$, $v \in \V{P}$, and $k \in \Z_{\geq 0}$. Let $E_1$,~$E_2$ denote the edges of $P$ adjacent to $v$ and let $E$ denote the opposite edge to $v$. We define the \emph{diagram} $\Diag_k(P,v)$ to be the set of subsets of $N_\R$, which we define inductively. We insist that $P \in \Diag_k(P,v)$ such that $P \in \Diag_k(P,v)$.
%\begin{itemize}
%		\item $P$
%	\end{itemize}


%	 the pair $(\sP_k(P,v), \iota_{P,v,k})$ such that,
%	\begin{itemize}
%		\item $\sP_k(P,v)$ is a two-dimensional simplicial complex with $2k+1$ maximal cells, and;
%		\item $\iota_{P,v,k}\colon |\sP_k(P,v)| \rightarrow \R^2$ is a continuous map from a geometric r%ealisation of $\sP_k(P,v)$ to $\R^2$. %non-convex
%	\end{itemize}
%	Denote the images under $\iota_k$ of chambers of $\sP_k(P,v)$ by $\fu_0$,~$\fu_{i,j}$ for $i \in \{1,2\}$ and $ 1 \leq j \leq k$. The complex $\sP_k(P,v)$ is determined by requiring that
%	\begin{enumerate}
%		\item the triangles $\fu_{i,j}$ meet along the following edges,
%		\begin{itemize}
%			\item[$\circ$] $\fu_{i,j}\cap \fu_{i,j-1}$ for $1 \leq j \leq k$
%			\item[$\circ$] $\fu_{i,1}\cap \fu_0$; and,
%		\end{itemize}
%		\item every chamber $\fu_{i,j}$ contains the distinguished vertex $v$.
%	\end{enumerate}
%	We fix the map $\iota_{P,v,k}$ by requiring that,
%	\begin{itemize}
%		\item $\iota_{P,v,k}\colon \fu_0 \rightarrow P$ isomorphically.
%\item Up to scale and translation $\iota_{P,v,k}(\fu_{i,1})$ is equal to the mutation of $P$ with mutating edge $E_i$ and fixed edge $E_{3-i}$.
%\item For $1 \leq j \leq k$, up to scale and translation $\iota_{P,v,k}(\fu_{i,j})$ is equal to the mutation of the Fano polygon corresponding to $\fu_{i,j-1}$ with mutating edge $E_{a_{i,j}}$ and fixed edge $E$. Here $a_{i,j}$ is defined by the requirement that $a_{i,j+1} = 3 - a_{i,j}$ and $a_{i,0} = i$.
%	\end{itemize}


%Having fixed the behaviour of the normal vectors to the new rays we record them using a pair of vectors $u^{(1)}_k$,~$u^{(2)}_k \in M$. These correspond to the rays `1' and `3' in Figure~\ref{fig:adding_rays}. For the upper sequence $v^{(1)}_j$ 



%We now prove a bound -- Lemma~\ref{lem:slope_bound} -- which ensures that the subset of the rays $\fe_i$ which lie in the region outside the cone formed by $\d_{1,\infty}$ and $\d_{2,\infty}$ is the union of edges of chambers $\fu_{i,j}$, as shown in Figure~\ref{fig:adding_rays}. This bound makes use of the fact that $P$ has singularity content $(3,\emptyset)$. Our first step is to relate the triple of weights $(a_1,a_2,a_3)$ determined by $P$ to the numbers $\ell_1$, $\ell_2$, and $s$.

$P_{(a,b,c)}$ is the Fano polygon corresponding to the Markov triple $(a,b,c)$, and $v$ is the vertex of $P_{(a,b,c)}$ corresponding to $a$


\begin{proof}[Proof of Proposition~\ref{prop:no_overlap}]
	There is an obvious partial order on $\Region(P)$: given $\fu,\fu' \in \Region(P)$ we say that $\fu \leq \fu'$ if for every $k$ such that $\fu' \in V_k(P)$ we have that $\fu \in V_k(P)$. TO DO: If $\fu' > \fu$, $\fu' \in R_\fu$. If $\fu$ is not comparable with $\fu'$ $R_\fu$ and $R_{\fu'}$ are (almost) disjoint.  In fact both these statements follow directly from Proposition~\ref{prop:better_bound}.
\end{proof}


%Given a chamber $\fu \in \Region(P)$, recall that $\fu = S_\fu(P_\fu)$ for a Fano polygon $P_\fu$ associated to a Markov triple $(b_1,b_2,b_3) \geq (a_1,a_2,a_3)$ and affine transformation $S_\fu$. Let $\fr^i_\fu$ denote the pair of rays $\fr^i$  Letting $\rho_\fu \colon \Z^2 \to M$ denote the map putting $P_\fu$ in standard form, we let $R_\fu$ be the subset $\rho_\fu^\star$

let $R_\fu$ be the subset of $\R^2$ bounded by the edge

If $P$ is associated to a Markov triple $(a,b,c)$, fixing a chamber $\fu \in \Region(P)$, we call the subset of $\R^2$ bounded by the edge $E$ and the rays XXX. It follows directly from Proposition~\ref{prop:better_bound} that $R_\fu$ is bounded in $\R^2$.


%\begin{proof}	
%	Mutate once backward and use the bound from  there. The following is old:	

%The chamber $\fu$ appears in $A_k$ for some $k \in \Z_{>0}$ as the image of the chamber $\fu^i_1$ in $\Diag_1(P_{\fu'},v_{\fu'})$ for some region $\fu'$. Figure~REF shows $P_{\fu'}$ in standard form with respect to $v$. We will show that the slope of the ray $\d$ in Figure~REF is greater than $g_{2,\infty}$, the slope of $\d_{2,\infty}$ emanating from $v_{\fu'}$. This bound is equivalent to the inequality $sc/z > g_{2,\infty}$. However, since $y/sb > g_{2,\infty}$ by Lemma~\ref{lem:slope_bound} it suffices to show that $sc/z > y/sb$. To do this we show that $z \leq sb$ and $y < sc$.
%\end{proof}

%	Note that $\Diag(P_\fu) \subset \Region(P_\fu)$ for any $\fu \in \Region(P)$, and each chamber $S_\fu(\Region(P_\fu)) \subset \Region(P)$. Let $k \in \Z_{\geq 0}$ be minimal such that $v \in \fu$ for some $\fu \in V_k$. Every chamber in $S_\fu\Diag(P_\fu)$ meets $v$, but any other $\fu' > \fu$ TO DO.

%Let $v \in \R^2$ be a vertex of a chamber in $\Region(P)$. Let $k \in \Z_{\geq 0}$ be minimal such that $v \in V_k$. If $v \notin \{v_1,v_2\}$, we have that $v$ is the vertex of a chamber $\fu \in V_k$ such that the corresponding vertex of $P_\fu$ is associated with the maximal value in a Markov triple. Replacing $P$ with $P_\fu$ we see that for any $\fu' \in \Diag(P,\rho)$, $\fu' \cap \rho^\star(P) = v := \rho^\star(v_3)$. Moreover $\fu'$ admits mutations to three chambers, two of which lie in $\Diag(P)$. Let $\fu'$ be the remaining chamber, and observe that $v_3 \notin R_{\fu'}$. Thus, any chamber greater than or equal to any chamber in $\Diag(P)$ does not meet $v$.

$V_v := \cl(\Phi_{v,v'}^{-1}(\Ima \Phi_{v,v'} \cap |\Region(P)|))$ where $v' \neq v$ is a choice vertex of $P$ which we suppress in the notation $V_v$, and 
\[
|\Region(P)| := \bigcup_{\fu : \fu \in \Region(P)}{\fu}
\]
is the \emph{support} of $\Region(P)$.


%TO DO: define $V \subset B^\vee_{\P^2}$ to be the gluing of these three and reword lemma $V_1$. We still need the definition of $W$ here, as well as the proofs that $W$ remains disjoint from $V$, and they `cover' $B^\vee_{\P^2}$.

%inductively constructing closed subsets $V_n \supset V_{n-1}$ covered by triangles corresponding to vertices of the trivalent graph $\mathcal{G}$ -- as defined on p.$3$ -- with distance $\leq n$ from the root vertex $(1,1,1)$ of $\mathcal{G}$. Defining $V := \lim_{n \geq 0}V_n$ we show that the edges of triangles in $V$ form the support of the set of rays of a structure $\sS$ intersected with $V$. We then argue in Proposition~WHICH that the support of $\sS$ is dense in the complement of $V$, completing the proof of \ref{it:dense}.

%We recall that we defined $V_0$ to be the `central region' of the affine manifold $B^\vee_{\P^2}$ -- shown in Figure~\ref{fig:initial_lines} -- in \S\ref{sec:aff_mfld}. Throughout this section let $P \subset \R^2$ be the Newton polytope of $x+y+1/xy$ and observe that there is a canonical identification between the interior of $V_0$ and the interior of $P$, regarded as integral affine manifolds.



We define $V_k$ inductively via a collection $A_k$ of triangular regions of $B^\vee_{\P^2}$, together with a set of linear maps sending each element of $A_k$ to a Fano polygon. Once we have defined $A_k$ we define,
\[
V_k := V_{k-1} \cup \bigcup_{T \in A_k} T.
\]
To begin the induction we set $A_0 := V_0$ together with the canonical identification of $V_0$ with $P$, and
\[
A_1 := \{T_{i,v} : i \in \{1,2\}, v \in \V{V_0}\}.
\]
Let $E$ be the shared edge between $V_0$ and some $\fu := T_{i,v} \in A_1$. Note that there is a unique shear and translation $S_\fu$ which maps the Fano polygon $P_\fu$ obtained by mutating $P$ in the edge $E$, to $\Phi_E(\fu \cap U_E)$. It will be useful later to use the notation $\Phi_\fu := \Phi_E$, and $U_\fu := U_E$. The set $A_{k+1}$ is constructed as follows: for each $\fu \in A_k$ note (inductively) that $\fu$ shares an edge with a chamber $\fu'$ in $A_{k-1}$ and let $v_\fu$ denote the remaining vertex of $\fu$; as well as the corresponding vertex of $P_\fu$. We then define
\[
A_{k+1} := \big\{ \Phi_\fu^{-1} \circ S_\fu(\fu^i_1) : \fu \in A_k, i \in \{1,2\} \text{, where } \fu^i_1 \in \Diag(P_\fu,v_\fu,1) \big\}.
\]

\begin{remark}
	The definition of $A_k$ involves a small abuse of notation, and more correctly would be the set of triangles $\cl(\Phi_\fu^{-1} \circ S_\fu({\fu^i_1}^\circ))$, as some triangles of this form meet $B^\vee_{\P^2} \setminus U_\fu$. See Figure~\ref{fig:gluing_things}(b) for an illustration of this phenomenon.
\end{remark}

For each $\fu' \in A_{k+1}$, let $\fu$ and $i$ be such that $\fu' = \Phi_\fu^{-1} \circ S_\fu(\fu^i_1)$. Set $P_{\fu'}$ to be the Fano polygon associated to $\fu^i_1 \in \Diag(P_\fu,v_\fu,1)$ (obtained from $P_\fu$ by a mutation). Set $S_{\fu'} := S_\fu \circ S_i$, where $S_i$ is the map -- defined in the discussion above Lemma~\ref{lem:gluing_chambers} -- which sends $P_{\fu'}$ to $\fu^i_1 \in \Diag(P_\fu,v_\fu,1)$. Finally set $\Phi_{\fu'} := \Phi_\fu$ and $U_{\fu'} := U_\fu$.

%set $S_\fu$ to be the scale and translation sending $P_{\fu'}$ to $\fu^i_1$ in $\Diag(P_\fu,v_\fu,1)$

%Assume that we have defined $A_j$ for all $j \in \{1,\ldots, k-1\}$, such that for each $\fu \in A_j$ there is a unique $v_\fu \in \V{\fu}$ for which $v_\fu$ is not contained in $V_{k-1}$. Observe that this condition certainly holds for $A_1$.

%We fix a choice of $\fu_1 \in A_1$ and hence a chart $U_{\fu_1} := U_E$ via this choice of chamber.

%Given an element $\fu \in A_{k-1}$, let $\Phi_\fu$ be a chart on $B^\vee_{\P^2}$ containing $\fu$. By construction, each element $\fu$ of $A_{k-1}$ is associated with a Markov triple $(a,b,c)$, and Fano polygon $P_\fu$ such that the toric variety determined by the spanning fan of $P_\fu$ is the weighted projective space $\P(a^2,b^2,c^2)$. We define
%\[
%A_k := \big\{ \Phi_\fu^{-1} \circ \iota_1(\fu_{i,1}) : \fu \in A_{k-1} \big\}
%\]
%where we slightly abuse notation to allow $v_\fu$ to refer to both a vertex of $\fu$ and the corresponding vertex of $P_\fu$. Examples of this gluing process are shown in Figure~\ref{fig:gluing_things}.



%This should admit an easy proof once I know enough about $V$.
%\begin{proof}
%	
%	Fix a chamber $\fu \in \bigcup_{k \geq 0}{A_k}$ and consider the diagram $\Diag_l(P_\fu,v_\fu)$. From Construction~\ref{const:gluing_chambers} we have that every triangle $\Phi^{-1}_\fu \circ \iota_l(\fu_{i,j})$ appears in some $A_{k'}$ where $k' \geq k$ and $l \geq j$ are positive integers. See Definition~\ref{dfn:diagram} for the definition of the chamber $\fu_{i,j}$. In other words, every triangle corresponding to a chamber of $\Diag_k(P_\fu,v_\fu)$ appears in $A_l$ for some $l \in \Z_{\geq 0}$.
%	
%
%	By Proposition~\ref{prop:rays_and_triangles} all the rays obtained by extending edges of triangles
%	
%	Observe that -- by Proposition~\ref{prop:slope_bound} -- the extension of $\d_E$ beyond $V$ is contained in $W$. Since $V \cap W$ contains only a discrete set of points no further subdivision of $V$ is created by extending the rays $\d_E$ inside $B^\vee_{\P^2}$.
%	
%	We conclude by observing that joints of $\sS$ which are contained inside $W$ produce rays which are contained in $W$. To see this fix a triangular region $\fu$, and consider a ray $\d$ generated by the scattering diagram at $\fu$. By Proposition~\ref{prop:rays_and_triangles} and Proposition~\ref{prop:slope_bound} we have that the slope of $\d$ is such that once it enters $C_{v_{fu_1}}$ or $C_{v_{fu_2}}$ it does not leave; here $\fu_i$ for $i \in \{1,2\}$ are chambers such that $v_{\fu_i}$ are the vertices of $\fu$ different from $v_\fu$. Since $C_{v_{\fu_i}}$ is convex, the cone $C$ formed between any two rays in $C_{v_{\fu_i}}$ is contained in this cone. In particular the cone formed between $\d$ and any other ray $\d'$ in $C_{v_{\fu_i}}$ is contained in this cone. Since any (outgoing) ray generated by the scattering diagram at the apex of $C$ is contained in $C$, such rays are contained inside in $W$. The same argument shows that rays produced at joints formed by the intersection of rays contained in $W$ are contained in $W$.
%\end{proof}

%We are now in a position to compare the rays defined by the edges of triangles in $A_k$ for $k \in \Z_{> 0}\geq 0$ with the support of the compatible structure $\sS$ defined by scattering. Recall that we describe the support of the structure $\sS$ in Construction~REF. We show that every ray which intersects the interior of the region $V$ is a ray $\d_E$, for some edge $E$ of a triangle in $A_k$ for some $k \in \Z_{\geq 0}$.



%We now compare the collection of rays $\d'_E$ generated by edges $E$ of triangles in $A_k$ for $k \in \Z_{> 0}$ as a set of rays in $B^\vee_{\P^2}$ with the support of the compatible structure $\sS$.
%We recall that this is the support of the rays appearing in $\sS$ on $B^\vee_{\P^2}$ obtained from the initial structure described in \S\ref{sec:aff_mfld}. Recall that in Construction~REF we describe the support of the structure $\sS$. We show in Proposition~\ref{prop:rays_are_edges} that every ray which intersects the interior of the region $V$ is a ray $\d'_E$, for some edge $E$ of a triangle in $A_k$ for some $k \in \Z_{\geq 0}$. Note that, assuming Conjecture~\ref{conj:dense_with_rays}, $W$ is exactly the subset of $B^\vee_{\P^2}$ densely covered by rays. We now show that $V$ and $W$ meet only the vertices of triangles in $\bigcup_{k \geq 0}{A_k}$.


We define the region $V_1$ to be the union of $V_0$ and three triangles in $B^\vee_{\P^2}$, two of which are shown in Figure~$6.1$(a). More precisely,





We now prove another technical lemma, used in the proof of Proposition~\ref{pro:dense_complement}. This lemma shows that, the segment of $\fe_i$ between the chamber $\fu^i_1$ and the ray $\d^i_\infty$ can be made arbitrarily small by choosing a solution of the Markov equation with a sufficiently large value of $s$. Recall that $P$ is a Fano polygon corresponding to the Markov triple $(a_1,a_2,a_3)$ and $a_3$ is a maximal value.

\begin{lem}
	\label{lem:vanishing_segment}
	Fix a value of $\epsilon \in \R_{> 0}$ and let $\ell(\fe_i)$ be the Euclidean length of the segment
	\[
	\fe_i \cap \bigcup^k_{j > 1} \fu^i_j.
	\]
	There is a value $\bar{s} \in \Z$ such that, if $s > \bar{s}$, then $\ell(\fe_i)/s \leq \epsilon$ for any $i \in \{1,2\}$ and $k \in \Z_{>0}$.
\end{lem}
\begin{proof}
	In the proof of Lemma~\ref{lem:slope_bound} we observed that the slope of $\fe_1$ is equal to $m := \frac{\ell_1}{s\ell_1-\ell_2}$. By Lemma~\ref{lem:standard_scale} the horizontal edge of $\fu_0$ -- see Figure~\ref{fig:adding_rays} -- has length $sa_2 = s\ell_2$. Moreover, from the proof of Lemma~\ref{lem:slope_bound} we have that the slope of $\fe_1$ is $\frac{\ell_1}{s\ell_1-\ell_2} $, hence the ray $\fe_1$ meets the vertical edge of $\fu^1_1$ at the point
	\[
	(0,y) := \left(0,\frac{s\ell_1\ell_2}{s\ell_1 - \ell_2}\right).
	\]
	We recall from Lemma~\ref{lem:comparison} that $s = 3a_3$. Let $y := \frac{s\ell_1\ell_2}{s\ell_1 - \ell_2}$ and observe that $\frac{s}{y} = \frac{s}{\ell_2} - \frac{1}{\ell_1}$. Substituting the expressions obtained in Lemma~\ref{lem:comparison}, $\frac{s}{y} = \frac{3a_3}{a_1} - \frac{1}{a_2} \geq 2$. Hence $y \leq \frac{s}{2}$ as $(a_1,a_2,a_3)$ ranges over integral solutions of the Markov equation. Since $y = \ell_2ms \leq \frac{s}{2}$, and $\ell_2 \geq 1$, we have that $m \leq \frac{1}{2}$.
	
	By Lemma~\ref{lem:asymptote_slope}, the slope of the ray $\d^i_\infty$ is $m^1_\infty > \frac{\bar{s}}{2}$. The length of the segment of $\fe_1$ between $(0,y)$ and the point of intersection with $\d^1_\infty$ is bounded by the length of a segment with one endpoint equal to $(0,\frac{s}{2})$, slope $\frac{1}{2}$, and the other end point on the line with slope $\frac{\bar{s}}{2}$. Calculating the Euclidean length of this segment we obtain the bound
	\[
	\ell(\fe_1) < \frac{\sqrt{5}s}{2(\bar{s}-1)},
	\]
	from which the result follows.
\end{proof}


%Note that, endowing the tree $\mathcal{G}$ of Markov triples with the partial order determined by distance from $(1,1,1)$, there is an element of $\Region(P)$ for every Markov triple greater than or equal to the triple corresponding to the polygon $P$. %Equivalently, given $\fu,\fu' \in \Region(P)$ we say that $\fu \leq \fu'$ if for every $k$ such that $\fu' \in V_k(P)$ we have that $\fu \in V_k(P)$.


%As shown in Figure~\ref{fig:gluing_things}, the construction of $V_k$ from $V_{k-1}$ in Definition~\ref{dfn:region} prolongs every edge which meets a vertex $v_\fu$ for some $\fu \in A_{k-1}$ for $k>1$. Since every edge of a triangle in $A_k$ which is not an edge of a triangle in $A_{k-1}$ meets a vertex $v_\fu$ for some $\fu \in A_k$, every edge $E$ is indefinitely prolonged to a ray $\bar{\d}_E$ inside $V$. Moreover -- as shown in Figure~\ref{fig:gluing_things}(a) -- the images of the triangles in $\Diag_1(P,v)$ in $B^\vee_{\P^2}$ extend the edges of $P$.

%Fixing a positive integer $k$ and a triangular region $\fu \in A_k$, let $C_\fu$ be the (irrational) cone in $B^\vee_{\P^2}$ generated by $\Phi^{-1}_\fu(\d_{i,\infty})$ for $i \in \{1,2\}$. We recall that for each diagram $\Diag_k(P,v)$, the rays $\d_{i,\infty}$ are the asymptotes toward which edges of the regions $\fu_{i,j}$ converge as $j \to \infty$. Similarly we define $W_0$ to be the union of the three cones $C_v$ defined as above, based at each vertex $v$ of $V_0$. Note that $C_v$ is contained in the domain of a chart $\Phi_{v,v'}$ for either vertex $v'$ of $V_0$ different from $v$. We will show in Lemma~\ref{lem:V_W_disjoint} that $V \cap W$ consists of the vertices of triangles in $V$, and show in Proposition~\ref{pro:dense_complement} that $V \cup W = B^\vee_{\P^2}$.

%	\begin{figure}
%		\includegraphics[scale=0.8]{region_between.pdf}
%		\caption{The region $R_\fu$ formed by two cones in $W$}
%		\label{fig:region_between}
%	\end{figure}


If $v_i$ is not a vertex of $P$ we define $C_{v_i}$ to be the cone $C_{\fu_i}$ where $\fu_i$ is the unique triangle such that $v_{\fu_i} = v_i$. If $v_i$ is a vertex of $P$, we define $C_{v_i}$ to be the cone -- as in the definition of $W_0$ -- formed between the asymptotes of the scattering diagram at $v_i$ in a chart $U_{v_i,v'}$ for some $v' \in \V{P}$.

	First note that the ray formed by extending the edge between $v_1$ and $v_\fu$ does not leave $C_{v_2}$ after it enters, by Lemma~\ref{lem:slope_bound}. Similarly the ray formed by extending the edge between $v_2$ and $v_\fu$ does not leave $C_{v_1}$ after it enters. In other words, 
	
	% We let $\bar{C}_\fu$ be the cone in $\R^2$ generated by the rays $\d^i_\infty$ for $i \in \{1,2\}$; the asymptotes which appear in the construction of $\Diag(P_\fu)$. We let $C_\fu := \Phi_{v,v'} \circ S_\fu(\bar{C}_\fu)$ be the the image of this irrational cone in $B^\vee_{\P^2}$, where $v' \in \V{P}$ is a vertex different from $v$. We set $W := XXX$
	
	% For each $v \in \V{P}$ and $\fu \in \Region(P,v) \setminus \{P\}$, let $\bar{C}_\fu$ be the cone in $\R^2$ generated by the rays $\d^i_\infty$ for $i \in \{1,2\}$, the asymptotes which appear in the construction of $\Diag(P_\fu)$. We let $C_\fu := \Phi_{v,v'} \circ S_\fu(\bar{C}_\fu)$ be the the image of this irrational cone in $B^\vee_{\P^2}$, where $v' \in \V{P}$ is a vertex different from $v$. Moreover we define $C_v$ to be the cone $\Phi_{v,v'}(\bar{C}_v)$ where $\bar{C}_v$ is the cone in $\R^2$ based at $v$ and with generated by rays $\d^i_\infty$, asymptotes of edges appearing in $\Diag(P,v)$. We now define $\cW$ to the be set of these cones, that is,
	
	
	\[
	\cW := \left\{C_\fu : \fu \in \Region(P) \right\} \cup \left\{ C_v : v \in \V{P}  \right\},
	\]
	and set $W := \bigcup_{C \in \cW}{C}$.
	
	 %In particular any ray which starts at a point $p$ in the half space defined by $E$ in $\R^2$ which does not contain $P$ in a direction $u$ which pairs negative with the inner normal to $E$ is contained in $U_{v,v'}$
	
	%	 (TO DO: move this somewhere) To this end, consider the region $R_\fu$ formed between the cones $C_{v_i}$ for $i \in \{1,2\}$ based at the vertices $v_1$ and $v_2$ respectively.
	
	 For $i \in \{1,2,3\}$ let $C_{v_i}$ be the cone in $\cW$ based at the vertex $v_i$ of $\fu$ shown in Figure~\ref{fig:comparison}.

	
% In the latter case $e_i \to 0$ as the lengths of all edges of $\fu_i$ approach zero.

%the image of the segment of $\fe_i$ considered in Lemma~\ref{lem:vanishing_segment} under a linear map. the composition of the map $(\rho^\star)^{-1}$ putting the  and the map sending XXX a segment of the ray $\fe_i$. Indeed TO DO: fix this linear map $A$. Note that as the Markov triple varies, the norm of the $sA$ remains bounded as the length of the edges of a Fano polygon in standard form a bounded below by $s$, and the image of any such triangle lies in a bounded region $R_\fu$ for some element $\fu \in A_1$. Since there exists a uniform bound on the norms of the linear maps $sA$, the length of the corresponding triangular region containing $x$ converges to zero by Lemma~\ref{lem:vanishing_segment}.


%We now prove another technical lemma, used in the proof of Proposition~\ref{pro:dense_complement}.

%\begin{lem}
%	Let $z$ be the length of the horizontal segment between $v$ and $\fr_2$, as illustrated in Figure~\ref{fig:better_bound}. For any $\epsilon \in \R_{> 0}$ there is a $\bar{s} \in \Z$ such that if $s > \bar{s}$, $z < \epsilon s$.
%\end{lem}
%\begin{proof}
%	This is a variant of the argument used in the proof of Proposition~\ref{prop:better_bound}. 
%\end{proof}


% Note that only three of the eight charts $\Phi_{v_1,v_2}$ are needed to cover $B^\vee_{\P^2}$.% To simplify notation later we choose three charts $\Phi_E \in \{\Phi_{v_1,v_2} : v_1, v_2 \in \V{V_0}\}$ such that $E$ is the edge of $V_0$ whose vertices are $v_1$ and $v_2$. We also let $U_E$ denote the domain of $\Phi_E$.

%\begin{remark}
%	\label{rem:ray_choices}
%	Note that the requirement that $v \in U_v$ only fixes which ray to remove emanating from \emph{two} of the focus-focus singularities (see Figure~\ref{fig:gluing_things}), we make the choice of ray to remove emanating from the third singularity arbitrarily -- it will play no role in what follows.
%\end{remark}

	%Assume first that $\fu' > \fu$. By Lemma~\ref{lem:containment} $\fu' \subset R_{\fu''}$ for some successor $\fu''$ of $\fu$ in $\Region(P)$. However $R_{\fu''} \cap C_{\fu} \subset \{v_\fu\}$ and so by hypothesis these are disjoint.
	
	% In the region between these asymptotes there are non-zero functions supported on rays of any rational slope.
	
	%There is an obvious parallel to be drawn with the collection of rays we considered from the mutating family of triangles in Section~\ref{sec:diagrams}. In particular outside the region defined by the two asymptotes the recursive formulae for generating the support of the rays are identical.
	
	
	%\begin{figure}
	%	\includegraphics[scale=0.8]{comparison.pdf}
	%	\caption{Cones in $W$}
	%	\label{fig:comparison}
	%\end{figure}
	
	Thus moving between  Since the superpotential is manifestly algebraic in $P$ -- and equal to $x+y+1/xy$ --
	
	TO DO: line edit this.
	For every $k \geq 0$ the chambers contained in $U_k$ are stable (that is, they undergo no further subdivision as $k$ increases) we combine this with the discussion of broken line counting in Section~\ref{sec:GS_background} to conclude that, since the superpotential is manifestly algebraic in the central chamber $P$ of $U$ and the functions attached to each rays are of the form $1+z^m$, the effect of the wall crossing formula is precisely an algebraic mutation. Since all Laurent polynomial mirrors to $\P^2$ are obtained by mutating from the polynomial $x+y+\frac{1}{xy}$ and by Theorem~\ref{thm:superpotential} we can exhibit any sequence of mutations of this polynomial by wall crossings have proved Theorem~\ref{thm:superpotential_2}.
	
	
	There is a \emph{compatible structure}$\sS$ on $\breve{B}$ obtained via the Gross--Siebert reconstruction algorithm. The structure $\sS$ determines, for each $k$, a polyhedral decomposition $\sP_k$ of $\breve{B}$, and we write $\Chambers(\sS,k)$ for the set of maximal cells of $\sP_k$.
	
	
	
	%We prove Theorem~\ref{thm:superpotential} by gluing together three copies of $\Region(P)$ -- where $P$ is the central region in $\breve{B} := \breve{B}_{\P^2}$ -- which intersect along $P$, see Figure~\ref{fig:initial_lines}. We argue that the edges form a set of rays equal to the support of a collection of scattering diagrams and that the region dense with rays fills out the complement of the union of these collection of triangles.
	
	% Indeed, as a subset of $\R^2$, $(\Ima \Phi_{v,v'} \cap \fu)$ is independent of the (binary) choice of $v'$ for all $\fu \in \cV_v$.
	
	
	 
	
	refines the polyhedral decomposition $\sP$ to $\sP_k$, adding polyhedral objects called \emph{walls}\footnote{In the two-dimensional case these are also called \emph{rays}.} $\d$ which are equipped with functions $f_\d$. The algorithm creates new walls for each $k \in \Z_{\geq 0}$ and for a given $k$ the collection of walls and slabs is called a \emph{structure} $\sS_k$. The process of subdivision at each order defined in~\cite{GS1} ensures that the structure is, in the terminology of~\cite{GS1}, \emph{compatible}. 
	
	%Fix regions $\fu,\fu' \in \cT$. If $v_{\fu'}$ is a vertex of $\fu$ then $v_{\fu'} = C_{\fu'} \cap \fu$. Thus $V \cap W$ contains every vertex of a triangle in $\cT$. The result follows from the claim that $\fu \cap C_{\fu'}  = \varnothing$ for all $\fu' \in \cT$ such that $v_{\fu'} \notin \fu$.
	
	
	%	We recall that we can associate a quiver to the triangle $P$ whose nodes are in bijection with the edges of $P$, and there are $\det(\rho(E_1), \rho(E_2))$ arrows between the nodes corresponding to $E_1$ and $E_2$ respectively. Mutations of $P$ are compatible with mutations of this quiver, see \cite{KNP15} for details. Comparing the description of quiver mutation with the mutation of solutions to the Markov equation we see that $s = 3a_3$.
	
	\footnote{We recall from~\cite{GS1} that an \emph{exponent} is a section of an extension of the local system (away from $\Delta$) of integral tangent vectors $\Lambda$ by the constant sheaf $\underline{\Z}$. For an exponent $m$, let denote $\bar{m}$ denote the image of $m$ in $\Lambda$.}
	
	The data of $(B_{\P^2},\sP)$ together with the log structure determines an initial structure, $\sS[0]$. Following the Gross--Siebert algorithm we make use of various scattering diagrams to construct structures $\sS[k]$ for each $k$. In fact,in \S\ref{sec:proof}, we compute a collection of regions using mutation of polygons and argue using Proposition~\ref{prop:rays_and_triangles} that this is the support of the union of scattering diagrams, away from a region densely filled with rays.
	
	%, and that $I^{-1}(P)$ consists of three copies of $P \subset \breve{B}$. The fact that $I^{-1}(P)$ is three copies of $P$ follows immediately
	
	
	%	 Since the sets $R_E$ intersect in vertices of $P$, and $R_E \setminus U_{v,v'} \subset E$, 
	
	%	By Lemma~\ref{lem:edges_in_region} we have that triangles $\fu \in \Region(P,v)\setminus\{P\}$ form a set of rays in a domain in $\R^2$. Each such ray $\d$ is contained in $R_{\fu^i_1}(P)$ for some $i \in \{1,2\}$, and hence its image in $\breve{B}$ is contained in $R_E$ for some edge $E = \conv{v,v'}$ of $P$. Since $R_E \setminus U_{v,v'} \subset E$, $\d$ defines a ray in $R_E$, and hence in $V\cap R_E$. Moreover, every edge of $P$ is the edge of a triangle $\fu \in \Region_v\setminus{P}$ for some $v \in \V{P}$..
	
	 that rays in $C_{\fu}$ do not leave $C_{v_1}\cup C_{v_2}$ once they enter. In other words we have
	 
	 
	 %	Fixing regions $\fu, \fu' \in \cT$, the result follows from the claim that $\fu \cap C_{\fu'} \subset \{v_{\fu'}\}$. We first consider the claim for triangles $\fu'$ comparable with $\fu$. Note that -- up to part of an edge of $P$ -- $\fu$ and $\fu'$ are contained in a some chart $U_{v,v'}$ of $\breve{B}$. Given that $\fu' > \fu$ -- and regarding $\fu$ and $\fu'$ in the image of a chart $\Phi_{v,v'}$ -- we have that $C_{\fu'}$ is contained in the quadrant in $\R^2$ formed by extending the edges of $\fu$ incident to $v_\fu$. Thus $C_{\fu'} \cap \fu \subset \{v_\fu\}$, as required. If instead $\fu' < \fu$, then $\fu \subset R_{\fu''}$ for some successor $\fu''$ of $\fu'$. But it follows from the definition of $R_{\fu''}$ that $C_{\fu'} \cap R_{\fu''} = \{v_{\fu'}\}$.
	 
	 %	Fix vertices $v_1$ and $v_2$ of a pair of triangles in $\cT$. Note that, for each $i \in \{1,2\}$, $v_i$ is either a vertex of $P$, or equal to $v_{\fu}$ for some chamber $\fu \in \cT$. For each $i \in \{1,2\}$, set $\fu_i := P$ in the first case, and set $\fu_i := \fu$ in the second. The result follows from the claim that $\fu_1 \cap C_{v_2} \subset \{v_2\}$ for all choices of vertices $v_1$ and $v_2$. 
	 
	  and subject to the condition that, for any $\fu \in \cT$, there is a maximal cell $\sigma$ in $\sP_k$ such that $\fu \subseteq \sigma$. For example, for each $\fu \in \cT$ such that $d(\fu) = K$, consider a small rational enlargement $R'_\fu$ of $R_\fu$ such that $R'_\fu \setminus R_\fu$ is disjoint from $V$. Subdivide $R'_\fu$ by extending the edges of $\fu$ incident to $v_\fu$ in $R'_\fu$ (cf. rays $\d_{E_1}$ and $\d_{E_2}$ in  Figure~\ref{fig:vanishing}). Taking the four subsets of $R'_\fu$ obtained in this way to be maximal cells of $\sP_k$ extends $\sP_k$ over $V$. We are free to extend the decomposition arbitrarily over $\breve{B} \setminus V$, subject to the three conditions specified by \cite[Definition~$6.24$]{TropGeom}
	  
	  %Define  by insisting that $\fu \in \cT$ is an element of $\sP_k$ if $d(\fu) \leq K$, and taking an arbitrary extension of this decomposition (meeting the above three conditions) to $\breve{B}$ subject to the condition that, for any $\fu \in \cT$, there is a maximal cell $\sigma$ in $\sP_k$ such that $\fu \subseteq \sigma$.
	  
	  .
	  
	  Similarly, the rays generated at intersection points $x$ also satisfy the hypotheses of Lemma~\ref{lem:in_W} we have that 
	  
	   -- and regarding $\fu$ and $\fu'$ in the image of $\Phi_{v_1,v_2}$ --
	   
	   
	   %Fixing any $\fu \in \cT$, and setting $\fu' := \fu^1_1(P_\fu)$, there is the map $S_{\fu'}\colon x \mapsto \lambda x + u$ sending $P_{\fu'}$ onto $\fu'$. Recall from the proof of Proposition~\ref{prop:better_bound} that $\lambda \leq 1/2$. 
	   
	   Letting $\ell$ and $\ell'$ denote the lengths of the edges of $\fu_i$ and $\fu'_i$ corresponding to the common edge of $P_{\fu_i}$ and $P_{\fu'_i}$, we have that $\ell' \leq \frac{1}{2}\ell$
	   
	   	%We have two cases as $i \to \infty$: either one edge (and one entry in the corresponding Markov triple) is eventually constant; or the lengths of two edges -- and hence all edges -- of $\fu_i$ approach zero. In the former case observe that -- setting $\fu = \fu_i$ -- $e_i = \ell$ is the length of the image under $S_{\fu_i}$ of the edge of $P_{\fu_i}$ which is fixed by mutation, and hence decreases (at least) exponentially.
	   	
	   	Using the stronger bound for $\lambda$, if the smallest entry in $\ba$ is at least $K$, then $x \leq sa_1\frac{\lambda}{1-\lambda} \leq \frac{sa_1}{3K-2}$.
	   	
	   	the length of $\rho^\star\circ S_{\fu_i}(E_{3-j(i)})$ is at most $\frac{sa_1}{3K-2}$. However, the maps $A_i := S^{-1}_{\fu_i}\circ(\rho^\star)^{-1}$ send segments of length $sa_1$ and $sa_2$ to $E_1(i)$ and $E_2(i)$. Since both $E_1(i)$ and $E_2(i)$ are contained in the bounded region $R_{\fu_1}$, there is a uniform upper bound $L$ on $s|A_i|$. That is $s|A_i(v)| \leq L|v|$. Hence $e_i = |E_{3-j(i)}(i)| \leq L$	
	   	
	   	%	Observe that, for each $i \in \Z_{>0}$, $\fu_{i+1}$ is the image of the triangle $\fu'_i := \fu^{j(i)}_1(P_{\fu_i})$ under the map $S_{\fu_i}$ for some $j(i) \in \{1,2\}$. Let $S_i \colon x \mapsto \lambda x + u$ be the map sending $P_{\fu_{i+1}}$ onto $\fu'_i$; and recall from the proof of Proposition~\ref{prop:better_bound} that $\lambda \leq 1/2$. We have two cases as $i \to \infty$, depending on whether the minimal entry in $\ba_i$ forms a bounded sequence. In the first $j(i)$ is eventually constant. In this case $E_{3-j(i)}(i+1) \leq E_{3-j(i)}(i)/2$ for all sufficiently large $i \in \Z_{> 0}$. In the second case, for any $K \in \Z_{> 0}$, every entry in $\ba_i$ is at least $K$ for sufficiently large $i$. Fix a large value of $i$ such that $j(i+1) \neq j(i)$. It follows from the discussion on page $14$ that the length $|E_{j(i+1)}(i+1)|$ is at most $|E_{(3-j(i))}(i)|/(3K-1)$. Recall that $E_{j(i+1)}(i+1)$ is a shared edge of $\fu_{i+1}$ and $\fu_{i+2}$. Since every triangle $\fu_i$ is contained in the bounded region $R_{\fu_1}$, lengths of the edges of $\fu_i$ and $\fu_{i+1}$ are uniformly bounded by some $L \in \R$. Hence the maximal edge length of $\fu_{i+2}$ is bounded above by $x := 2L/(3K-1)$. The maximal edge length of $\fu_i$ is not necessarily decreasing as $i \to \infty$, however -- by repeated application of the triangle inequality -- we can show that the maximal of the edge length is uniformly bounded by $2L/(3K-2)$.
	   	
	   	
	   	
	   	%	Let $E_1(i)$ and $E_2(i)$ denote the edges of $\fu$ incident to $v_\fu$ and let $e_1(i)$ and $e_2(i)$ denote their respective lengths. Let $\Gamma$ be the cone formed at $v_\fu$ by the rays $\d_{E_1(i)}$ and $\d_{E_2(i)}$. Note that $x$ must lie in $\Gamma$, since $R_\fu \setminus \Gamma \subset V$. Let $X_i$ be the connected component of $(C \cap R_\fu) \setminus C_\fu$ which contains $x$, see Figure~\ref{fig:vanishing}. Observe that $X_i$ intersects $\fu_{i+1}$ in an edge of $\fu_{i+1}$. Two edges of $X_i$ are in $W$, while the remaining edge of $X_i$ extends an edge of $\fu_i$. Noting that $\fu$ is obtained from the Fano polygon $P_\fu$ by the affine transformation $S_\fu$, it follows from Remark~\ref{rem:small_seg} that this edge of $X_i$ has length shorter than the length of the edge if $\fu_i$ that it extends. It suffices to check that the lengths of these edges converge to zero as $i \to \infty$.
	   	
	   	
	   	
	   	%Let $b \colon \Z_{> 0} \to \{1,2\}$ be such that $\fu_i \cap \fu_{i+1} = E_{b(i)}(i)$ for each $i > 0$, and let $(e_1(i),e_2(i))$ denote the lengths of edges $\fu_i$ not shared with $\fu_{i-1}$.
	   	
	   	
	   	$e_{b(i+1)}(i+1) \leq e_{b(i)(i)}/2$ for all sufficiently large $i$.
	   	
	   	Assume instead that the minimal entry in $\ba_i$ is unbounded; choose an integer $K > 1$, and a value of $i$ such that $b(i+1) \neq b(i)$ and all entries in $\ba_i$ are bounded below by $K$. Observe that, since $\fu_i$ and $\fu_{i+1}$ are contained the bounded region $R_{\fu_1}$ the lengths of their edges have a uniform upper bound $L \in \R$. From the discussion on page~$14$ we have that $e_b(i+1)(i+1) \leq e_{3-b(i)}(i)/(3K-1)$. Since $b(i+1) \neq b(i)$ we have that both  $e_1(i+2)$ and $e_2(i+2))$ are bounded above by $x := L/(3K-1)$. The sequences $e_1(j)$ and $e_2(i+2))$ need not be decreasing for $j > i$, but we observe from repeated application of the triangle inequality that $e_1(j)$ and $e_2(j)$ are bounded above by $L/(3K-2)$ for all $j \geq i+2$. Indeed, the edge lengths $e_1(j)$ and $e_2(j)$ are bounded by
	   	
	   	that $e(j)$ and $f(j)$ are bounded above by $2L/(3K-2)$ for all $j \geq i+2$. Indeed, the edge lengths $e(j)$ and $f(j)$
	   	
	   		
	   	
	   	Each such ray $\d$ is either contained in $V \cap R_E$ for some edge $E = \conv{v,v'}$ of $P$, or contains an edge of $P$. In the first case the map $\Phi^{-1}_{v,v'}$ identifies the ray $\d$ with a ray in $V$. In the second we observe that the complement of an initial segment is contained in $R_{E'}$, for some edge $E'$ of $P$, and hence also defines a ray in $V$.
